A Continuous Risk Assessment Methodology for Cloud Infrastructures

Cloud systems are dynamic environments which make it difficult to keep track of security risks that resources are exposed to. Traditionally, risk assessment is conducted for individual assets to evaluate existing threats; their results, however, are quickly outdated in such a dynamic environment. In this paper, we propose an adaptation of the traditional risk assessment methodology for cloud infrastructures which loosely couples manual, in-depth analyses with continuous, automatic application of their results. These two parts are linked by a novel threat profile definition that allows to reusably describe configuration weaknesses based on properties that are common across assets and cloud providers. This way, threats can be identified automatically for all resources that exhibit the same properties, including new and modified ones. We also present a prototype implementation which automatically evaluates an infrastructure as code template of a cloud system against a set of threat profiles, and we evaluate its performance. Our methodology not only enables organizations to reuse their threat analysis results, but also to collaborate on their development, e.g. with the public community. To that end, we propose an initial open-source repository of threat profiles.

==> sections/background.tex <==
!TEX root = ../continuous-risk-assessment.tex

\subsection{Risk Assessment}
In this section, we describe the traditional risk assessment process that we used as a basis for our own proposal.
%
We loosely base our description on the NIST guidelines for risk assessment \cite{blank2011guide} %, highlighting parts of the process that are essential to our own risk assessment process. The approach described here is asset-centric 
% other threat modeling approaches may instead focus on the attacker or the software \cite{shostack2014threat} but are not considered here.
which can be divided into four phases: \textit{preparation}, \textit{threat analysis}, \textit{impact analysis}, and \textit{risk calculation}. % also the work of Torr \cite{torr2005demystifying}

\subsubsection{Preparation}
In the first phase, the assessment is prepared by defining the basic conditions, e.g. identifying the scope of the assessment, identifying underlying assumptions, and defining the risk assessment model to be used. This model also describes the capabilities of the attacker.
Furthermore, the relevant assets are identified and their protection goals are defined. As protection goals, confidentiality, integrity, and availability (CIA) are commonly considered, possibly extended by authenticity, authorization, and non-repudiation.

\subsubsection{Threat analysis}
In this phase threats are identified. 
% , e.g. to the confidentiality of a virtual machine or to the integrity of a storage container
Often, graphical representations, like attack trees or attack graphs, are used to depict the attack paths that can lead to a successful attack on a certain protection goal of a certain asset. In quantitative approaches concrete probability values for certain attacks, or leaf nodes of an attack tree, are assessed on a predefined scale.

When evaluating the threat level for an attack tree, i.e. the probability of a successful attack against one protection goal of one asset, the attack path with the highest probability, i.e. the attack path that is easiest to implement for the attacker, is applied to the attack tree as a whole. % This means that the leaf nodes are evaluated and then propagate upwards according to \textit{or} and \textit{and} conditions.
Note that attack paths may also reference other attack trees, for example an attack path on the integrity of a blob storage may reference the integrity attack tree of a function which has write-access to the blob storage. % This way, complex attack paths can be modeled.
%In Section~\ref{use_case} we show, e.g., how a storage container's integrity can be attacked via a serverless function that has write-access to the container. This way, sophisticated attack paths can be modeled.
%
Figure~\ref{fig:attacktree} shows a simplified attack tree that a threat analysis may develop for such a blob storage. 

\begin{figure}
\begin{center}
\includegraphics[width=0.7\linewidth, keepaspectratio]{figures/attacktreeStorageAccount.png}
\caption{A simplified example attack tree for the integrity of a generic cloud blob storage. The rightmost leaf node indicates a reference to another attack tree that shows attack paths on the integrity of a serverless function.}
\label{fig:attacktree}
\end{center}
\end{figure}

\subsubsection{Impact analysis}
In this phase, the potential impacts that could result from a successful attack are evaluated per protection goal and asset. Impact dimensions may include financial damage, reputation damage, and loss of privacy. Again, these dimensions may be quantified by the risk assessment experts and merged to an impact score per asset and protection goal.

\subsubsection{Risk calculation}
Finally, a risk score is calculated using the results of the threat and impact analyses. One commonly used way to calculate a risk score is to multiply the values for the threat probability and the corresponding impact value for each protection goal of an asset.
The resulting risk values can then be used to prioritize and visualize the risks. % , and to determine mitigations 

Consider what such a process means for a cloud system: The assets that are assessed may include various resources whose configurations may change frequently. A risk assessment would therefore be outdated quickly since even one modified configuration, like a changed port number, can open up new attack paths on a number of resources. Also, new assets may be created frequently which could also have an impact on other resources. At the same time, the identified attack paths are similar across resources and across organizations that use the same cloud provider making them potentially reusable.


==> sections/use_case.tex <==
%!TEX root = ../continuous-risk-assessment.tex

In the following we describe a use case for Module 1 of our risk assessment process. Thereafter, we describe our prototype implementation for Module 2. %, and discuss the limitations and effectiveness of our approach.

Consider the following scenario. Company \textit{CloudControl} operates a cloud service that allows its customers to remotely control their smart home devices, e.g. to switch on the heating remotely or to monitor the power consumption. It is composed of several virtual machines, virtual networks, storage containers, as well as serverless functions. % that scale automatically with the occurring workload. % TODO add more flexibility and "dynamics"

% Ontology approach: Note that in this use case description, we leave out detailed descriptions of the preparation, and the assessment of threat and impact values, since these are standard risk assessment steps which are not special in our approach, as described in Section~\ref{background}.
The protection goals that CloudControl considers are confidentiality, integrity, and availability. They furthermore pursue a quantitative risk assessment and define the risk 
model as follows. Threat levels, as well as impact values, are quantified in the interval $[1,3]$ for each protection goal of an asset. Risk values are then calculated by multiplying threat and impact value for a certain protection goal, resulting in the interval $[1,9]$. The risk for a certain asset and protection goal is calculated using the highest threat level of all branches that are identified for a particular combination.
%(in Section~\ref{background} we have explained how attack probabilities propagate through an attack tree). 

% Let $R(a_p)$ denote the risk value for an asset $a$ and its protection goal $p$. Let furthermore $Threat(tp_i, a_p)$ denote the threat level of the threat profile $tp$ for the protection goal $p$ of an asset $a$, then:
% \begin{equation}
% R(a_p) = max(Threat(TP, a_p)) * Impact(a_p)
% \label{equ:risk}
% \end{equation}

% CloudControl then sets up the necessary tooling for Module 2.

CloudControl prepares the continuous risk assessment process and performs the Module 1 activities \textit{identify configuration weaknesses}, \textit{create threat profiles}, and \textit{assess threat and impact values} (see Section~\ref{module1}) as described in the following.

\subsubsection{Identify configuration weaknesses}
CloudControl uses a publicly available repository of threat profiles as the basis for their own risk assessments. CloudControl's security experts review the public repository once a month and adapt the configured threat levels according to their own evaluation.

During this monthly review, one new threat profile is identified. This threat profile increases the minimum TLS version that is considered secure for all resources that offer a TLS configuration, since a vulnerability has been found in the old version. 
% TODO reintegrate? The security experts know that CloudControl still relies on the old TLS version, but integrate the new threat profile nevertheless to make the respective threat visible in their continuous risk assessment so risks can be taken into account and mitigations can be identified.

During the review it also becomes clear that Azure Web Apps are being used as a new resource type. A threat assessment for this asset type results in two new branches. The first branch concerns the availability of the Web App. Since it scales automatically, CloudControl sets a limit to how much cost it can consume which in turn results in a resource exhaustion threat if an attacker is able to generate enough requests to make the Web App reach that cost limit. The second branch results from the Web App having write-access to a Storage Account, i.e. a new branch in the respective Storage Account's integrity attack tree. Note that this branch could easily extend to further resources which may access the Storage Account's data and process it which could be described in threat profiles as shown in the following. % TODO these branches are ported to CWs defined in threat profiles
% They reference the integrity attack tree of the Web App since a compromised Web App can result in a compromised Storage Account.


\subsubsection{Create threat profiles}
In this activity, missing threat profiles are created for every identified CW. These are stored in a local repository that is later used by the Module 2 implementation. 
Listing~\ref{lst:policy} shows the threat profile related to the required TLS version. Note that this profile will be applied to all resources that offer the respective TLS configuration, including Storage Accounts and Web Apps in our example.
\begin{lstlisting}[
    basicstyle=\scriptsize,
    label={lst:policy},
    caption={A simplified threat profile described in Rego. It checks for all resources of the type \textit{storageAccount} if they have not set TLS1.2 as the minimum required version and returns their names (see the following section for more Rego examples).},
    keywordstyle=\bfseries,
    % morekeywords={storageaccount_confidentiality_eavesdrop, split},
    captionpos=b,
    belowskip=0.2 \baselineskip
]
all_confidentiality_abuseVulnerableTLSVersion[insecure_endpoints] {
  resources[i].properties.minimumTlsVersion != "TLS1_2"
  insecure_endpoints := resources[i].name
}
\end{lstlisting}

% Ontology approach: cut back
\subsubsection{Assess threat and impact values}
% In the final Module 1 activity, CloudControl assesses threat and impact values for the the identified attack paths and the assets' protection goals. 
%
To assesses threat and impact values, CloudControl assesses the attack probability of each CW, as well as possible financial impact, the reputation damage, and the possible loss of privacy for customers when a certain asset's protection goal is compromised. 

The new attack path regarding the vulnerable TLS version is assessed with a probability of $1$ (low), since an attack abusing the vulnerability is deemed unlikely. The probability of a denial of service attack on the Web App, however, is assessed with a probability value of $2$ (medium).
%
The new Web App asset is assessed with an impact value of $1$ (low) for its availability, and a value of $3$ (high) for its confidentiality and integrity, since it does not affect critical business processes, but it may process personal customer data.  

CloudControl decides to conduct a further assessment after one month. In this follow-up assessment, the security staff will pursue two goals: First, it will evaluate whether significant differences have occurred in the cloud architecture, e.g. if new asset types have been created, that should trigger a new execution of Module 1. Second, it will review the shared threat profile repository to identify new contributions that are relevant to CloudControl's own cloud system and integrate these into their local threat profile DB.

We have published the threat profiles\footnote{For the final version of this paper, we will publish the source code and threat profiles and include a link here.} of this use case (as well as further threat profiles) so they can be used as a shared threat profile repository. The repository also includes the source code of our prototype implementation which we present in the following section.


